On-the-Fly Coding to Enable Full Reliability Without Retransmission

This paper proposes a new reliability algorithm specifically useful when retransmission is either problematic or not possible. In case of multimedia or multicast communications and in the context of the Delay Tolerant Networking (DTN), the classical retransmission schemes can be counterproductive in terms of data transfer performance or not possible when the acknowledgment path is not always available. Indeed, over long delay links, packets retransmission has a meaning of cost and must be minimized.In this paper, we detail a novel reliability mechanism with an implicit acknowledgment strategy that could be used either within these new DTN proposals, for multimedia traffic or in the context of multicast transport protocols. This proposal is based on a new on-the-fly erasure coding concept specifically designed to operate efficient reliable transfer over bi-directional links. This proposal, named Tetrys, allows to unify a full reliability with an error correction scheme. In this paper, we model the performance of this proposal and demonstrate with a prototype, that we can achieve a full reliability without acknowledgment path confirmation. Indeed, the main findings are that Tetrys is not sensitive to the loss of acknowledgments while ensuring a faster data availability to the application compared to other traditional acknowledgment schemes. Finally, we pave the first step of the integration of such algorithm inside a congestion controlled protocol.

==> implement.tex <==
\section{Implementation issues}
\label{sec:implement}

In the previous sections, we have illustrated through real measurements and simulations the feasibility of the concept proposed. From these results, several points related to the implementation of the mechanism must be discussed.

The first one is the the size of the finite field. This point was presented in the previous Section where it has been shown that the size of a finite field must be at least of $8$.

The second point deals with the loss patterns and the packet loss rate in the channel. It has been shown that when the repair ratio is larger than the packet loss rate, the mechanism correctly performs. However, the decoding delay can be large. In the case of real-time applications, the repair ratio can be tuned in order to obtain decoding delays smaller than the maximum delay acceptable by the application. Note that the packet loss rate and the model of the 2-states Markov channel can be updated during the transmission \cite{yajnick:infocom99}.

Another important point concerns the patterns of repair packets at the sender side. Indeed, in the modelling and the simulations, we have just fixed the repair ratio. Actually, it can be observed that the performance of the mechanism can be significantly improved if the repair packets are sent in a regular interval. For example, for a packet loss rate of $0.1$ over a Bernoulli channel, with repair packets randomly sent with a rate $0.1667$, the mean decoding delays is equal to $33.30$. On the same channel, if the sender repeats the following pattern: one repair packet sent every 5 source packets, the repair ratio is still $0.1667$, but the observed mean decoding delays is equal to $15.88$. 

The complexity is also a point that must be carefully evaluated. Two kinds of operations must be performed by the decoder. First, it has to subtract the received source packets to the received repair packets. This operation can be performed on-the-fly as soon as a repair packet is received. Note that the average number of packets that must be subtracted depends on the recurrence time. The second operation is the matrix inversion and the multiplication of the matrix by the repair packets to recover the source packets. For a $m\times m$-matrix, the inversion is done in $O(m^3)$ operations and the multiplication of the matrix by the packets needs $O(sz.m^2)$ operations, where $sz$ is the number of symbols of the finite field in each packet. 
Clearly, the amount of computations depends on the recurrence time and matrix size. Since these parameters depends on the difference between the packet loss rate and the repair ratio, we can establish a direct relation between the amount of computations and the repair ratio. Consequently, a device constrained in energy can enlarge the repair ratio in order to reduce the amount of computations.

